KAT-Coder Technical Report

Recent advances in large language models (LLMs) have enabled progress in agentic coding, where models autonomously reason, plan, and act within interactive software development workflows. However, bridging the gap between static text-based training and dynamic real-world agentic execution remains a core challenge. In this technical report, we present KAT-Coder, a large-scale agentic code model trained through a multi-stage curriculum encompassing Mid-Term Training, Supervised Fine-Tuning (SFT), Reinforcement Fine-Tuning (RFT), and Reinforcement-to-Deployment Adaptation. The Mid-Term stage enhances reasoning, planning, and reflection capabilities through a corpus of real software engineering data and synthetic agentic interactions. The SFT stage constructs a million-sample dataset balancing twenty programming languages, ten development contexts, and ten task archetypes. The RFT stage introduces a novel multi-ground-truth reward formulation for stable and sample-efficient policy optimization. Finally, the Reinforcement-to-Deployment phase adapts the model to production-grade IDE environments using Error-Masked SFT and Tree-Structured Trajectory Training. In summary, these stages enable KAT-Coder to achieve robust tool-use reliability, instruction alignment, and long-context reasoning, forming a deployable foundation for real-world intelligent coding agents. Our KAT series 32B model, KAT-Dev, has been open-sourced on https://huggingface.co/Kwaipilot/KAT-Dev.

==> sections/Reinforcement-to-Deploymen.tex <==
\section{Reinforcement-to-Deployment Adaptation: Bridging Research Agents and Real-World Workflows}

Existing datasets for code agents in the supervised fine-tuning (SFT) stage are primarily derived from research-oriented frameworks such as SWE-Agent, which rely on linear, single-session dialogues and homogeneous operation pipelines. While these datasets are effective for controlled academic evaluation, they fail to capture the complexity of real-world agentic environments.

In practical software engineering, agents must operate within heterogeneous toolchains, dynamically manage long-horizon dependencies, and adapt to non-linear conversational trajectories involving frequent context switches and multi-turn reasoning. This gap between research benchmarks and production-grade workflows leads to a significant distribution mismatch, limiting the generalization ability of agentic code models when deployed in real development systems.

\paragraph{Data Construction across Production Environments}
To bridge this research–deployment gap, we construct a new generation of Agentic Workflow training data by integrating our early-stage KAT-Coder models with production-grade IDE-based systems such as Claude Code, Cline, Roo Code, and CodeFlicker. These environments offer realistic execution traces, tool invocations, and iterative human–agent interactions, enabling the construction of data that reflects true software development dynamics.

This integration yields trajectories that are far more diverse and realistic but also introduces new training challenges.

\paragraph{Training Challenges in Production-Grade Trajectories}
Production workflows differ substantially from benchmark settings in two major aspects:
(1) \textbf{Expanded Tool Spectrum} — Real-world agents interact with dozens of heterogeneous tools (e.g., debuggers, linters, package managers), leading to frequent erroneous or redundant tool calls.
(2) \textbf{Non-Linear Context Boundaries} — Compression checkpoints, context truncation, and mode switches (e.g., between coding, planning, and execution) introduce branching points that disrupt the continuity of dependency chains.

These challenges make direct imitation learning unstable, as gradient propagation from noisy tool calls or broken trajectories can degrade convergence and overfit to spurious behaviors.

\paragraph{Methodology: Error-Masked SFT and Tree-Structured Trajectory Training}
To address these issues, we adopt two complementary strategies designed for agentic fine-tuning under complex tool and context dynamics:
(1) \textbf{Error-Masked SFT (EM-SFT)}: We leverage execution feedback logs to identify tool-use failures and selectively mask gradients from erroneous tool calls. This prevents error amplification during backpropagation while retaining the model’s exposure to self-corrective reasoning signals.
(2) \textbf{Tree-Structured Trajectory Training (TST)}: We decompose multi-branch trajectories into locally coherent subtrees defined by context compression boundaries and mode transitions. Within each subtree, standard supervised fine-tuning is performed independently, ensuring stable optimization and improved temporal consistency.

Together, these strategies enable the policy model to learn from realistic, production-grade trajectories without sacrificing training stability or semantic coherence. This forms the foundation for aligning the model’s behavior with human engineering workflows—an essential step toward fully deployable agentic coding systems.


==> sections/architecture.tex <==
\section{Architecture}
